Detecting and Learning Out-of-Distribution Data in the Open world: Algorithm and Theory

This thesis makes considerable contributions to the realm of machine learning, specifically in the context of open-world scenarios where systems face previously unseen data and contexts. Traditional machine learning models are usually trained and tested within a fixed and known set of classes, a condition known as the closed-world setting. While this assumption works in controlled environments, it falls short in real-world applications where new classes or categories of data can emerge dynamically and unexpectedly. To address this, our research investigates two intertwined steps essential for open-world machine learning: Out-of-distribution (OOD) Detection and Open-world Representation Learning (ORL). OOD detection focuses on identifying instances from unknown classes that fall outside the model's training distribution. This process reduces the risk of making overly confident, erroneous predictions about unfamiliar inputs. Moving beyond OOD detection, ORL extends the capabilities of the model to not only detect unknown instances but also learn from and incorporate knowledge about these new classes. By delving into these research problems of open-world learning, this thesis contributes both algorithmic solutions and theoretical foundations, which pave the way for building machine learning models that are not only performant but also reliable in the face of the evolving complexities of the real world.

==> README <==
This is a dissertation template for UW Madison. It builds on
memoir.cls (which you'll need to have installed) and on the (venerable
but subtly-broken) withesis.cls.  You'll want to process your document
with pdflatex.  For best results, you'll want the following packages
installed somewhere in your TEXINPUTS as well:

* amssymb
* amsmath
* hyperref
* theorem

(Note that none of these are required, and that you can comment out
any of those packages if you don't need to use them.)

This package is included in the distribution, but you can use your own
if you have a version more recent than 2007/06/30:

* enumitem

The following packages are used if you have them, but you can comment
them out if you don't need/want them:

* microtype
* natbib
* mathpartir
* booktabs
* svn-multi

I suggest making one subdirectory for each chapter, and putting
the .tex file and all of the figures for that chapter there.
Then, simply \include each chapter in dissertation.tex.

By default, your pages and chapter headings should be set up to
conform to the UW typesetting requirements.  If you are making a
version of your dissertation that doesn't require conformance to
typewriter-era requirements (e.g. for the web or to make a nice
printed copy), you'll want to create your own page and chapter styles
in includes/preamble.tex and change frontmatter/frontmatter.tex to
select your styles instead of the "deposit" styles.

Other files of interest include:

 * backmatter/colophon.tex: if you're a big nerd and want to tell
   everyone the excruciating details of your typesetting
   adventures, this is the place.

 * frontmatter/abstract.tex:  your abstract goes here

 * frontmatter/acks.tex:  your acknowledgements go here

 * frontmatter/frontmatter.tex: sets up the main structure for
   the front matter of your diss

 * includes/defs.tex: your commands/environments; includes one
   for epigraphs at the beginning of chapters and one for
   per-file SVN info

 * includes/preamble.tex: this is where you want to set up your
   chapter and page styles (see the excellent memoir class
   documentation on CTAN) and include any other packages you need

 * includes/thesisdefs.tex: some definitions adapted from the withesis
   document class

This template is basically unsupported, but you should feel free to
email me questions -- just know that I might not be able to deliver
a timely or useful reply.  (On the other hand, I absolutely welcome
patches that provide fixes or functionality enhancements.)

For your convenience, this template includes two files that are not in
some LaTeX distributions.  Both are covered under the terms of the
LPPL; if you have a more recent version of either file, just delete
the included versions.  (Note that the "hanglist" environment for
nicely-typeset enumerated lists depends on a fairly recent version of
enumitem.)

 * mcbride.bst is copyrighted by Chung-chieh Shan
 * enumitem.sty is copyrighted by Javier Bezos

Again, these are available from CTAN and are only included here for
your convenience.  If your local LaTeX installation has recent
versions of these files, please 

The definitions in defs/thesisdefs.tex are adapted from withesis.cls,
which is licensed under the Perl Artistic License and is also
available from CTAN.

Good luck!


Will Benton
Madison, WI  2008

ps: see http://web.willbenton.com/writing/2008/better-latex


==> backmatter/colophon.tex <==
\svnidlong{$LastChangedBy$}{$LastChangedRevision$}{$LastChangedDate$}{$HeadURL: http://freevariable.com/dissertation/trunk/frontmatter.tex $}
\vcinfo{}

This template uses Gyre Pagella by default.  (I used Arno Pro in my dissertation.)

Feel free to give me a shout-out in your colophon or acks if this template is useful for you.  Good luck!

